Zero-shot Object-Centric Instruction Following: Integrating Foundation Models with Traditional Navigation

Large scale scenes such as multifloor homes can be robustly and efficiently mapped with a 3D graph of landmarks estimated jointly with robot poses in a factor graph, a technique commonly used in commercial robots such as drones and robot vacuums. In this work, we propose Language-Inferred Factor Graph for Instruction Following (LIFGIF), a zero-shot method to ground natural language instructions in such a map. LIFGIF also includes a policy for following natural language navigation instructions in a novel environment while the map is constructed, enabling robust navigation performance in the physical world. To evaluate LIFGIF, we present a new dataset, Object-Centric VLN (OC-VLN), in order to evaluate grounding of object-centric natural language navigation instructions. We compare to two state-of-the-art zero-shot baselines from related tasks, Object Goal Navigation and Vision Language Navigation, to demonstrate that LIFGIF outperforms them across all our evaluation metrics on OCVLN. Finally, we successfully demonstrate the effectiveness of LIFGIF for performing zero-shot object-centric instruction following in the real world on a Boston Dynamics Spot robot.

==> chapters/data-association.tex <==
\subsection{Probabilistic Data Association in SLAM}

==> chapters/intro_icra.tex <==
\section{Introduction}
\label{sec:intro}

% Robots assisting humans with household chores, elderly care, and search and rescue operations has become increasingly popular over the past decade. The most intuitive way for humans to interact with these robots is through natural language. With significant advancements in natural language understanding, computer vision, and robotics, there is growing interest in the research community to develop robots capable of comprehending human language and executing instructions accordingly. In this work, we explore how capable a robot is of following natural language navigation instructions in an unseen unexplored indoor environment. This task is particularly challenging since the robot needs to ground the language instructions to the visual observations and make intelligent decisions to follow the route specified in the instruction.

Significant advancements in natural language understanding, computer vision, and robotics have led to a growing interest in the research community to develop robots capable of comprehending human language and executing instructions accordingly. Benchmarks created to drive progress towards this goal often group multiple distinct challenges into a single task, making it difficult to study specific reasoning capabilities independently of one another. In this work, motivated by both human navigation behavior and established approaches to robotics, we propose a new dataset to investigate object-centric navigation instruction following in robots. %The core challenge of this dataset is in how to ground the language instructions to the visual observations in a way that allows the robot to determine both where it is in the instruction and which direction in the environment corresponds to the next part of the instruction.

Humans perform visual navigation by using landmarks to determine where they are in the world. Landmarks are distinctive sites in a scene such as objects or topological features (e.g., a particular tree or building). While we can understand relative movement from our current location (e.g., move 5 meters forward), grounding this spatial understanding in landmarks is required to understand our placement in larger regions% (e.g., now I am by the front door)
~\cite{object_important, janzen2004selective, foo2005humans, schinazi2010neural}. 
%https://www.ncbi.nlm.nih.gov/pmc/articles/PMC3866451/#RSTB20120533C1
%https://www.cmor-faculty.rice.edu/~cox/neuro/HCMComplete.pdf
To follow navigation instructions, humans associate landmarks described in natural language with real landmarks observed in the environment to simultaneously understand where they are in the instruction and in the world. 
%In this work, we investigate landmark-based instruction following in robots.

%Clear natural language navigation instructions require references to these landmarks, and performing successful landmark-based navigation requires localization respect to landmarks.  

Roboticists studying mapping and navigation have developed methods for creating landmark maps from visual observations and using those maps for autonomous navigation~\cite{thrun2006graph, mur2017orb, campos2021orb, rosinol2020kimera,rosinol2021kimera,labbe2019rtab,placed2023survey}. In fact, work in this area has matured far enough to move beyond the research community. Landmark-based mapping and navigation systems are widely used for autonomous robot operation in many industry applications, including home robot vacuum cleaners~\cite{robotvacuum,eade2010monocular} and drones for surveying and inspection~\cite{drones}. With recent advances in natural language understanding due to large language and vision-language models~\cite{openai2023gpt4, li2023blip2, radford2021learning,liu2023grounding,kirillov2023segment}, the next frontier is to determine how to accurately align natural language navigation instructions with observation-based autonomous decision making capabilities in these mature robotic systems.

To support research in this direction, researchers have developed benchmarks for evaluating an autonomous agent's ability to follow natural language navigation instructions in simulation, specifically R2R~\cite{anderson2018vision}, RxR~\cite{ku2020room}, and VLN-CE~\cite{krantz2020beyond}. These benchmarks consist of datasets of natural language instructions and associated paths through scanned Matterport 3D scenes of residential homes~\cite{chang2017matterport3d}.
% These datasets contain two distinct navigation challenges. 
The language instructions in these datasets contain both object-centric references to landmarks (`move forward to the \textit{blue chair}, turn left and stop at the \textit{wooden table}') and relative positional references to the current agent position (`move forward and turn left and stop in the hallway'). 
% For example, `go to the blue chair, then turn left and stop at the wooden table' versus `move forward and turn left and stop in the hallway' respectively.
In contrast, we focus on the capability of object-centric instruction following alone. There is substantial value in disentangling these two challenges from both cognitive science and robotics perspectives. 
Neuroscience researchers have found that distinct regions of the brain enable people to perform landmark-based spatial navigation using observed objects~\cite{object_important}. 
While successful artificial intelligence algorithms are frequently not a direct mimic of human neural function, roboticists also have a long history of managing landmark-based navigation~\cite{durrant2006simultaneous} and relative positional navigation~\cite{sibley2010vast,sibley2009adaptive,anderson2015relative} with clearly distinct methodological approaches. This distinction in both biological systems and autonomous navigation algorithms suggests that effective language grounding for these two navigation types may require distinct approaches.

%To support research in this direction, researchers have developed benchmarks for evaluating an autonomous agent's ability to follow natural language navigation instructions in simulation, specifically R2R~\cite{anderson2018vision}, RxR~\cite{ku2020room}, and VLN-CE~\cite{krantz2020beyond}. These benchmarks consist of datasets of natural language instructions and associated paths through scanned Matterport 3D scenes from inside residential homes~\cite{chang2017matterport3d}. While methods trained on these datasets achieve high success rates in simulation, they are impractical on real robots due to sim-to-real gaps. Zero-shot approaches using state-of-the-art open-vocabulary object detectors show promise for real-world transfer but currently underperform on these benchmarks. This is partly because these detectors struggle with identifying larger spatial concepts like rooms and hallways, limiting their ability to handle commands not involving specific objects.

%The reliance on off-the-shelf open-vocabulary object detectors can limit our understanding of the true potential of VLN capabilities. To address this, our work poses a crucial question: ``What is the practical potential of current VLN technologies for real-world robotic applications if we assume ideal object detection capabilities?'' This inquiry aims to evaluate the core challenges of VLN independent of current detector limitations.

%To answer this question, we focus on two key areas: first, we investigate zero-shot methods with object-centric instruction following, exploring their effectiveness in generalizing to this new task without specific training. Second, we examine the feasibility of deploying these methods on physical robots, addressing the challenges of transferring simulated successes to real-world scenarios.

%By disentangling VLN capabilities from object detection limitations, this research aims to identify the strengths and weaknesses of current technologies and provide a clearer roadmap for advancing autonomous navigation systems that can effectively understand and execute complex, natural language instructions in diverse environments.


%Grounding natural language to more spatial ideas may require substantially different strategies than grounding them to landmark-based instructions. 

%quite successfully determined semantic mapping of landmarks and then regions separate from 

%These two observations lead us to hypothesis 
%This strategy, known as landmark-based piloting, contrasts with path integration strategies in which self-motion cues are used to determine displacement relative to a known starting position
%\todo{EXPLAIN}
%\todo{if there are evidence from robotics literature to indicates that VLN trained methods don't work well in the real world, it would be good to reference them.} \todo{These two zero-shot methods compared to some trained methods in the real world and the trained methods did badly: ~\cite{long2023discuss,xu2023vision}. Don't think there is are large-scale experiments showing a variety of trained methods do poorly in the real world though. For objectnav ~\cite{gervet2023navigating} showed that modular learned methods performed better in the real world than end-to-end.}

% NOTE this is a nice observation but kind of an aside and we can cut for space
%\textcolor{blue}{In addition, the evaluation criteria of these prior benchmarks is biased toward trained methods. To facilitate their metrics for success, abstract concepts in language are grounded to precise points in space on the path. For an agent to be ``successful" it must stop within a relatively small fixed radius of the labeled position. However, in our example ``move forward and turn left and stop in the hallway" anywhere in the hallway is a correct place to stop to follow the instruction, but existing benchmarks would only label a small region of the hallway as successful. As a result, many trained methods will learn labeling patterns of the dataset instead of learning an accurate mapping of language to observations yielding artificially high performance in these navigation scenarios. Object-centric navigation instructions remove much of this source of language grounding ambiguity and provide a fairer comparison on a scoped task.}

%But success is low, benchmarks combine 2 problems (landmark-based piloting and path integration) which are separately handled in human brains and working robot systems


%\cite{savva2019habitat,szot2021habitat}

\textbf{Contributions.} In this work, we present a novel instruction-following navigation dataset, \textit{\datasetname} (\datasetnameshort), including solely object-centric navigation instructions. We also propose \methodnamefull (\methodname), a novel method for grounding natural language object-centric instructions to robot observations and poses, while performing zero-shot navigation in unseen unexplored environments. 
% We present a novel navigation policy to actively perform \methodname in order to follow natural language instructions on \datasetnameshort. 
\methodname leverages pre-trained vision and language foundation models and require no task-specific training. Finally, we demonstrate the viability of \methodname to successfully perform real-world instruction following on a Boston Dynamics Spot robot.

==> chapters/method-graph-optim.tex <==
\subsubsection{Joint Optimization of Inferred and Observed Graphs}
At the beginning of each episode, we obtain the inferred pose graph from the language instruction (top half in \Cref{fig:method_fgraph_example}). Here $p_i$ and $o_i$ are the imagined robot poses and the objects respectively.
Suppose the instruction is ``Go forward to the piano and go past the table".
Like humans would imagine a graph in their head from this instruction alone, we too imagine the inferred graph to contain robot poses with $(p_{i_x}, p_{i_y}, p_{i_\theta})$, where $(p_{i_x}, p_{i_y})$ is the 2D position of $p_i$ and $p_{i_\theta}$ is its orientation (yaw). Such an inferred graph will then contain an initial pose $p_1$ and a second pose $p_2$ such that the factor $\phi(p_2,p_1)$ encodes the forward movement by an initial estimated amount (say, 5 meters). This will however have a high uncertainty in the forward direction, and low uncertainty in the other axes and orientation.
At the same time, we could say that the object/landmark, `piano' ($o_1$) is visible from the pose $p_2$. This also has an uncertainty associated with its pose, since it might not be exactly in front of the robot, but slightly left or right. 
The uncertainties are modeled as Gaussian noise with zero mean. This inferred graph is thus initialized at the beginning of the episode and is considered as a prior for the pose graph optimization as the robot navigates.

Next the robot starts the episode with an initial pose $x_1$ such that $\phi(x_1)$ is given as a prior. As the robot moves around, it observes landmarks $l_i$ and create nodes for every pose $x_i$, thus incrementally building the observed graph.
As the robot adds new poses $x_i$ to the observed graph, we optimize the whole graph (inferred + observed) jointly.
The optimization will then be equivalent to minimizing the following:
\begin{multline}
\label{eq:factor_graph_map}
    X^{MAP} = argmin_x \big[
    \sum_i ||h_i(x_i,l_i) - z_i(x_i,l_i)||^2_{\sum_i} \\
    + \sum_i ||h_i(x_i,p_i) - z_i(x_i,p_i)||^2_{\sum_i} \\
    + \sum_i ||h_i(p_i,o_i) - z_i(p_i,o_i)||^2_{\sum_i}
    \big]
\end{multline}

\input{figures/fig-method-fgraph-example}

where $h_i(x_i,l_i)$ is the measurement from a given pose $x_i$ to a landmark $l_i$, $h_i(x_i,p_i)$ is the measurement from the observed pose $x_i$ to the inferred pose $p_i$, and $h_i(p_i,o_i)$ is the measurement from the inferred pose $p_i$ to the inferred object $o_i$.

\todo{will there be a factor between the observed and inferred objects $h_i(l_i,o_i)$? if yes, then when will they be connected? we could do this -- if $sem\_similarity(l_i,o_i)$ is higher than a threshold, then create a factor $\phi(l_i,o_i)$.}.


==> chapters/method-waypoint-selection.tex <==
\subsubsection{Waypoint Selection}

At each time step, the agent will determine the waypoint ($W_i$) to navigate to, following this equation:
\begin{equation}
\label{eq:waypoint_selection}
    W_i = argmin_{p_j} [
    distance(x_i, p_j) - \lambda\eta(p_j)
    ] 
\end{equation}

Here, $p_j \in P=\{p_1,p_2,...\} $ is an inferred pose in the language-inferred graph, $x_i$ is the current robot pose, $\lambda$ is a hyperparameter for the uncertainty $\eta(p_j)$ on the position of the pose $p_j$.
Then \Cref{eq:waypoint_selection} means selecting the closest inferred pose to the robot for which the uncertainty is high. The idea is that the graph optimization in \Cref{eq:factor_graph_map} would have optimized all `seen' inferred poses and that the robot now needs to `find' the next inferred pose with high uncertainty.

==> chapters/preliminary.tex <==
\subsection{Preliminaries: Factor Graphs}
\label{sec:prelim_factor}

Factor graphs~\cite{koller2009probabilistic} are probabilistic graphical models~\footnote{\url{https://gtsam.org/tutorials/intro.html}} and are widely used to model complex problems in Robotics.
A factor graph is a bipartite graph consisting of variables, representing unknown random variables and factors, representing constraints on the variables. The factors are local in nature such that they are dependent on a subset of the entire set of variables. The entire factor graph then captures the global function of variables as a product of multiple local functions~\cite{dellaert2017factor}. Factor graphs can be used to model different estimation problems in Robotics, such as Simultaneous Localization and Mapping (SLAM). In our work, we specifically focus on pose graph optimization along with landmark measurements.

Formally, a factor graph is represented as $F = (U, V, E)$ where $U$ is a set of factors $\phi_i$, V is the set of variables $x_j$, and E are the edges $e_{ij}$ between the factors and variables nodes. 
$N(\phi_i)$ is the set of variable nodes adjacent to the factor $\phi_i$ and $\pose_i$ is an assignment to this set. Then the factor graph $F$ can be defined as the factorization of a global function $\phi(X)$ as:
\begin{equation}
\label{eq:factors}
    \phi(X) = \prod_i{\phi(X_i)}
\end{equation}

\mypara{Pose Graph.}
A factor graph can be used to represent a pose graph where the variables represent the robot poses ($\pose_i$), including position and orientation and the factors ($f_i$) are the odometry measurements between the poses. The pose $x_1$ is the initial pose which is considered a prior. Optimizing the factor graph then means finding the best set of poses that satisfy the odometry constraints as closely as possible.

\mypara{Pose Graph with Landmarks.}
A factor graph can also contain the observed landmarks ($\obslandmark_i$) as a second type of variables in addition to robot poses ($\pose_i$). The poses are connected by factors representing odometry measurement. A landmark and a pose are connected by a factor $fl_{i}$ representing the observation measurement. 
An example is shown in \Cref{fig:prelim_landmark_slam}, where each small black node is a factor and connected to the variables it depends on. 

\input{figures/fig-prelim-landmark-slam}

\mypara{Pose Graph Optimization in SLAM.}
Pose Graph Optimization~\cite{dellaert2017factor} in SLAM improves the predicted robot poses, while it moves through an environment. This is done by minimizing the error between the predicted and the observed poses by taking into consideration the relationships and constraints between the poses and the observed landmarks. 
Following \Cref{eq:factors}, we can write the example factor graph from \Cref{fig:prelim_landmark_slam} in terms of the following factorization:
\begin{equation}
\label{eq:factor_graph_example}
    \phi(l_1,l_2,x_1,x_2,x_3) = 
            \phi(x_1) \phi(x_2,x_1) \phi(x_3,x_2)
            \phi(x_1,l_1)\phi(x_2,l_1)
            \phi(x_3,l_2)
\end{equation}

It can be shown that maximum a posteriori (MAP) inference for SLAM with a Gaussian noise model is equivalent to solving a nonlinear least-squares problem (for details refer to \cite{dellaert2017factor}). 
Assuming all factors follow the following form with Gaussian noise:
\begin{equation}
\label{eq:factor_graph_gaussian}
    \phi(X_i) \propto 
            \exp \{
                -\frac{1}{2} ||h_i(X_i) - z_i||^2_{\sum_i}
            \},
\end{equation}
MAP inference is equivalent to minimizing a sum of nonlinear least-squares:
\begin{equation}
\label{eq:factor_graph_map}
    X^{MAP} = argmin_x \sum_i ||h_i(X_i) - z_i||^2_{\sum_i}
\end{equation}
where $h(.)$ is a measurement prediction function and the measurement from a given pose x to a landmark l is modeled by $z = h(x, l) + \eta$. Here $\eta$ is a noise drawn from a zero-mean Gaussian density. The measurement functions $h(.)$ is non-linear in the Robotics applications, since the odometry factors are non-linear consisting of the robot orientation.
Nonlinear optimization methods such as the Levenberg-Marquardt (LM) algorithm can then be applied to converge to the global minimum in \Cref{eq:factor_graph_map} through linear approximations.

% A way to estimate the robot poses is through maximum a posteriori (MAP). It maximizes the posterior density $p(X|Z)$ of the states $X=\{x_1,x_2,...\}$ given the measurements $Z=\{z_1,z_2,...\}$.

% \begin{equation}
% \label{eq:map_basic}
%     X^{MAP} = argmax_x~p(X|Z)
%             = argmax_x~\frac{p(Z|X)p(X)}{p(Z)}
% \end{equation}

% \Cref{eq:map_basic} can be written as \Cref{eq:map_refined}, by ignoring the normalization factor p(Z), since the measurements Z are given and p(Z) do not contribute to the maximization.

% \begin{equation}
% \label{eq:map_refined}
%     X^{MAP} = argmax_x~l(X;Z)p(X)
% \end{equation}

% Here, l(X;Z) is the likelihood of the states X given Z, which is proportional to $p(Z|X)$.

==> chapters/task.tex <==
\section{Task}
\label{sec:task}


==> figures/fig-dataset-features.tex <==
\begin{figure}[ht]
\centering
% \begin{subfigure}{\linewidth}
%   \centering
%   % include first image
%   \includegraphics[width=\linewidth]{figures/images/word_cloud_noun.pdf}  
%   \caption{}
%   \label{fig:sub-first}
% \end{subfigure}
% \begin{subfigure}{\linewidth}
%   \centering
%   % include first image
%   \includegraphics[width=\linewidth]{figures/images/word_cloud_all_words.pdf}  
%   \caption{}
%   \label{fig:sub-second}
% \end{subfigure}
\includegraphics[trim=90 35 90 35 0,clip,width=0.4\linewidth]{figures/images/word_cloud_noun.pdf}  
\includegraphics[trim=90 35 90 35 0,clip,width=0.4\linewidth]{figures/images/word_cloud_actions.pdf}  
\caption{
% \textbf{Dataset Features.} 
\datasetnameshort instructions feature a variety of common household objects (left) and action directives (right).
}
\label{fig:dataset_feature}
\vspace{-10pt}
\end{figure}

==> figures/fig-dataset-overview.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/images/dataset.pdf}
\caption{Dataset Overview. \todo{to be merged with Fig3 for teaser}}
\label{fig:dataset_overview}
\end{figure}

==> figures/fig-method-overview.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/images/method_overview.pdf}
\caption{Method Overview.}
\label{fig:method_overview}
\end{figure}

==> figures/fig-pose-representation.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.6\linewidth, trim = 0cm 6cm 12cm 0cm, clip]{figures/images/pose_representation.pdf}
\caption{
Pose representation -- all poses are represented by ($x,y,\theta$).
}
\label{fig:pose_repres}
\end{figure}

==> figures/fig-prelim-landmark-slam.tex <==
\begin{figure}[ht]
\centering
\begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
\node[main] (1) [fill = black] {};
\node[main] (2) [right of=1] {$x_1$};
\node[main] (3) [right of=2] [fill = black] {};
\node[main] (4) [right of=3] {$x_2$};
\node[main] (5) [right of=4] [fill = black] {};
\node[main] (6) [right of=5] {$x_3$};
% \node[main] (7) [right of=6] [fill = black] {};
\node[main] (8) [above of=4] [fill = black] {};
\node[main] (9) [above of=8] {$l_1$};
\node[main] (10) [above of=3] [fill = black] {};
\node[main] (11) [above of=6] [fill = black] {};
\node[main] (12) [above of=11] {$l_2$};
\draw (1) -- (2);
\draw (2) -- (3);
\draw (3) -- (4);
\draw (4) -- (5);
\draw (5) -- (6);
% \draw (6) -- (7);
\draw (4) -- (8);
\draw (8) -- (9);
\draw (2) -- (10);
\draw (9) -- (10);
\draw (6) -- (11);
\draw (11) -- (12);
\end{tikzpicture} 
\caption{Landmark-based SLAM}
\label{fig:prelim_landmark_slam}
\end{figure}


==> figures/fig-teaser.tex <==
\begin{figure*}[ht!]
\centering
\subfloat[Caption for first figure]{
    \includegraphics[width=0.28\textwidth]
    {figures/images/dataset.pdf}
}
\hfill
\subfloat[Caption for second figure]{
    \includegraphics[width=0.68\textwidth]{figures/images/method.pdf}
}
\caption{
\methodname
}
\label{fig:teaser}
\end{figure*}

==> figures/fig-waypoint-landmark-relation.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.6\linewidth, trim = 0cm 8cm 14cm 0cm, clip]{figures/images/waypoint_landmark_relation.pdf}
\caption{Waypoint-Landmark relation ($r_{\waypoint_{i},\inflandmark_{i}}$ in \Cref{eq:pose_optim}) explained.}
\label{fig:way_land_rel}
\end{figure}
